CAFO: Feature-Centric Explanation on Time Series Classification

In multivariate time series (MTS) classification, finding the important features (e.g., sensors) for model performance is crucial yet challenging due to the complex, high-dimensional nature of MTS data, intricate temporal dynamics, and the necessity for domain-specific interpretations. Current explanation methods for MTS mostly focus on time-centric explanations, apt for pinpointing important time periods but less effective in identifying key features. This limitation underscores the pressing need for a feature-centric approach, a vital yet often overlooked perspective that complements time-centric analysis. To bridge this gap, our study introduces a novel feature-centric explanation and evaluation framework for MTS, named CAFO (Channel Attention and Feature Orthgonalization). CAFO employs a convolution-based approach with channel attention mechanisms, incorporating a depth-wise separable channel attention module (DepCA) and a QR decomposition-based loss for promoting feature-wise orthogonality. We demonstrate that this orthogonalization enhances the separability of attention distributions, thereby refining and stabilizing the ranking of feature importance. This improvement in feature-wise ranking enhances our understanding of feature explainability in MTS. Furthermore, we develop metrics to evaluate global and class-specific feature importance. Our framework's efficacy is validated through extensive empirical analyses on two major public benchmarks and real-world datasets, both synthetic and self-collected, specifically designed to highlight class-wise discriminative features. The results confirm CAFO's robustness and informative capacity in assessing feature importance in MTS classification tasks. This study not only advances the understanding of feature-centric explanations in MTS but also sets a foundation for future explorations in feature-centric explanations.

==> Tabels/GI_full_measrue.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\centering
\fontsize{7}{8}\selectfont{
\begin{tabular}{cccccccccccc}
\hline
 &
   &
  \multicolumn{5}{c}{\textbf{GILON}} &
  \multicolumn{5}{c}{\textbf{MS}} \\ \cline{3-12} 
\multirow{-2}{*}{\textbf{Models}} &
  \multirow{-2}{*}{\textbf{Methods}} &
  \textbf{ABC($\uparrow$)} &
  \textbf{DACC($\uparrow$)} &
  \textbf{WDACC($\uparrow$)} &
  \textbf{$\rho_{\text{S}}(\uparrow)$} &
  \multicolumn{1}{c:}{\textbf{$\rho_{\text{K}}(\uparrow)$}} &
  \textbf{ABC($\uparrow$)} &
  \textbf{DACC($\uparrow$)} &
  \textbf{WDACC($\uparrow$)} &
  \textbf{$\rho_{\text{S}}(\uparrow)$} &
  \textbf{$\rho_{\text{K}}(\uparrow)$} \\ \hline
 &
  GS &
  0.1524 &
  -0.4518 &
  0.1954 &
  0.1051 &
  \multicolumn{1}{c:}{0.0813} &
  -0.1591 &
  {\color[HTML]{000000} 7.0145} &
  0.1668 &
  0.0514 &
  \textbf{0.0667} \\
 &
  SVS &
  0.8191 &
  0.0922 &
  0.3313 &
  0.1007 &
  \multicolumn{1}{c:}{0.0681} &
  0.2253 &
  {\color[HTML]{000000} \textbf{11.0621}} &
  0.3291 &
  -0.0686 &
  -0.0667 \\
 &
  Saliency &
  \textbf{1.1923} &
  \textbf{4.0154} &
  \textbf{0.5467} &
  {\color[HTML]{FF0000} \textbf{0.3710}} &
  \multicolumn{1}{c:}{\textbf{0.2571}} &
  0.0393 &
  {\color[HTML]{000000} -4.8612} &
  0.1422 &
  0.1029 &
  0.1467 \\
 &
  FA &
  0.7140 &
  0.3139 &
  0.3312 &
  0.1486 &
  \multicolumn{1}{c:}{0.1077} &
  {\color[HTML]{FF0000} \textbf{0.4919}} &
  {\color[HTML]{000000} 4.9340} &
  0.2876 &
  -0.0914 &
  -0.0400 \\
 &
  IG &
  0.2100 &
  -0.1184 &
  0.1934 &
  0.0457 &
  \multicolumn{1}{c:}{0.0330} &
  -0.0157 &
  {\color[HTML]{000000} -2.0845} &
  0.2410 &
  \textbf{0.0743} &
  \textbf{0.0667} \\
 &
  CE &
  0.6846 &
  3.3256 &
  0.4786 &
  0.2070 &
  \multicolumn{1}{c:}{0.1429} &
  0.3552 &
  {\color[HTML]{000000} 7.7819} &
  {\color[HTML]{FF0000} \textbf{0.4757}} &
  0.0629 &
  0.0133 \\
\multirow{-7}{*}{ShuffleNet} &
  \cellcolor[HTML]{EFEFEF}CE+QR(Ours) &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{1.2270}} &
  \cellcolor[HTML]{F2F2F2}{\color[HTML]{FF0000} \textbf{8.1576}} &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.7607}} &
  \cellcolor[HTML]{EFEFEF}\textbf{0.3525} &
  \multicolumn{1}{c:}{\cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.2703}}} &
  \cellcolor[HTML]{EFEFEF}\textbf{0.3376} &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{21.0326}} &
  \cellcolor[HTML]{EFEFEF}\textbf{0.4505} &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.6400}} &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.5467}} \\ \hline
 &
  GS &
  1.2847 &
  \textbf{3.9358} &
  {\color[HTML]{FF0000} \textbf{0.6716}} &
  \textbf{0.4532} &
  \multicolumn{1}{c:}{\textbf{0.3187}} &
  0.0595 &
  {\color[HTML]{FF0000} \textbf{8.4381}} &
  \textbf{0.3563} &
  0.0514 &
  0.0133 \\
 &
  SVS &
  0.5772 &
  0.8351 &
  0.2812 &
  0.1341 &
  \multicolumn{1}{c:}{0.1165} &
  0.1600 &
  {\color[HTML]{000000} 4.5203} &
  0.3443 &
  \textbf{0.3600} &
  \textbf{0.2800} \\
 &
  Saliency &
  {\color[HTML]{FF0000} \textbf{1.3389}} &
  2.6527 &
  \textbf{0.6631} &
  0.3644 &
  \multicolumn{1}{c:}{0.2879} &
  0.1542 &
  {\color[HTML]{000000} \textbf{8.3272}} &
  0.3455 &
  0.2514 &
  0.2000 \\
 &
  FA &
  0.8476 &
  0.1180 &
  0.4409 &
  -0.0145 &
  \multicolumn{1}{c:}{- 0.0242} &
  {\color[HTML]{FF0000} \textbf{0.3507}} &
  {\color[HTML]{000000} 7.0373} &
  {\color[HTML]{FF0000} \textbf{0.3732}} &
  0.1086 &
  0.0667 \\
 &
  IG &
  \textbf{1.2895} &
  2.1370 &
  0.6204 &
  \textbf{0.4532} &
  \multicolumn{1}{c:}{\textbf{0.3187}} &
  -0.0058 &
  {\color[HTML]{000000} 7.9354} &
  0.2443 &
  0.0514 &
  0.0133 \\
 &
  CE &
  0.8010 &
  1.5534 &
  0.4204 &
  0.3705 &
  \multicolumn{1}{c:}{0.2703} &
  \textbf{0.1758} &
  {\color[HTML]{000000} -0.6670} &
  0.0077 &
  -0.0629 &
  -0.0667 \\
\multirow{-7}{*}{ResNet} &
  \cellcolor[HTML]{EFEFEF}CE+QR(Ours) &
  \cellcolor[HTML]{EFEFEF}1.1636 &
  \cellcolor[HTML]{F2F2F2}{\color[HTML]{FE0000} \textbf{6.3932}} &
  \cellcolor[HTML]{EFEFEF}0.6150 &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.5815}} &
  \multicolumn{1}{c:}{\cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.4418}}} &
  \cellcolor[HTML]{EFEFEF}0.1179 &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} 1.2667} &
  \cellcolor[HTML]{EFEFEF}0.2544 &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.4400}} &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.3333}} \\ \hline
 &
  GS &
  -0.3077 &
  0.4944 &
  0.1122 &
  0.2308 &
  \multicolumn{1}{c:}{0.1560} &
  0.2949 &
  {\color[HTML]{000000} 2.5729} &
  0.2187 &
  -0.0400 &
  0.0133 \\
 &
  SVS &
  -0.7084 &
  3.3303 &
  0.0632 &
  0.1648 &
  \multicolumn{1}{c:}{0.1121} &
  {\color[HTML]{FF0000} \textbf{0.3286}} &
  {\color[HTML]{000000} 3.9830} &
  0.2261 &
  -0.1371 &
  -0.1200 \\
 &
  Saliency &
  0.9861 &
  3.4468 &
  0.4908 &
  {\color[HTML]{FF0000} \textbf{0.5253}} &
  \multicolumn{1}{c:}{{\color[HTML]{FF0000} \textbf{0.4110}}} &
  0.3216 &
  {\color[HTML]{FF0000} \textbf{6.6423}} &
  \textbf{0.2634} &
  \textbf{0.0400} &
  \textbf{0.0400} \\
 &
  FA &
  0.4570 &
  1.0416 &
  0.2698 &
  -0.0651 &
  \multicolumn{1}{c:}{-0.0462} &
  0.3005 &
  {\color[HTML]{000000} 3.2092} &
  0.2260 &
  -0.0457 &
  -0.0133 \\
 &
  IG &
  -0.3012 &
  0.7879 &
  0.1157 &
  0.2352 &
  \multicolumn{1}{c:}{0.1692} &
  \textbf{0.3263} &
  {\color[HTML]{000000} 2.7889} &
  \textbf{0.2631} &
  -0.0400 &
  0.0133 \\
 &
  CE &
  \textbf{0.9202} &
  {\color[HTML]{FF0000} \textbf{8.1179}} &
  \textbf{0.5312} &
  \textbf{0.3305} &
  \multicolumn{1}{c:}{\textbf{0.2396}} &
  0.1257 &
  {\color[HTML]{000000} 0.7309} &
  0.1653 &
  -0.1429 &
  -0.0933 \\
\multirow{-7}{*}{MLP-Mixer} &
  \cellcolor[HTML]{EFEFEF}CE+QR(Ours) &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{1.1442}} &
  \cellcolor[HTML]{F2F2F2}\textbf{8.1057} &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.6975}} &
  \cellcolor[HTML]{EFEFEF}0.1657 &
  \multicolumn{1}{c:}{\cellcolor[HTML]{EFEFEF}0.1297} &
  \cellcolor[HTML]{EFEFEF}0.2763 &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} \textbf{6.0934}} &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.2890}} &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.9086}} &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.8133}} \\ \hline
 &
  GS &
  -0.1973 &
  1.2441 &
  0.1161 &
  0.2185 &
  \multicolumn{1}{c:}{0.1473} &
  \textbf{0.1690} &
  {\color[HTML]{000000} 5.2190} &
  0.3615 &
  {\color[HTML]{FF0000} \textbf{0.3600}} &
  {\color[HTML]{FF0000} \textbf{0.2800}} \\
 &
  SVS &
  -0.6079 &
  \textbf{2.8303} &
  0.0839 &
  0.1314 &
  \multicolumn{1}{c:}{0.0813} &
  {\color[HTML]{FF0000} \textbf{0.1821}} &
  {\color[HTML]{000000} \textbf{5.2272}} &
  0.3186 &
  -0.0400 &
  -0.0667 \\
 &
  Saliency &
  \textbf{0.5871} &
  1.2168 &
  0.3764 &
  0.1204 &
  \multicolumn{1}{c:}{0.0989} &
  0.1227 &
  {\color[HTML]{000000} 5.2190} &
  0.3291 &
  0.0514 &
  0.0400 \\
 &
  FA &
  0.2449 &
  0.3672 &
  0.2230 &
  - 0.0541 &
  \multicolumn{1}{c:}{-0.0242} &
  {\color[HTML]{FF0000} \textbf{0.1821}} &
  {\color[HTML]{000000} \textbf{5.2272}} &
  0.3186 &
  0.1429 &
  0.1200 \\
 &
  IG &
  -0.1767 &
  1.2441 &
  0.1199 &
  0.2004 &
  \multicolumn{1}{c:}{0.1385} &
  0.1690 &
  {\color[HTML]{000000} 5.2190} &
  0.3615 &
  \textbf{0.1771} &
  \textbf{0.1733} \\
 &
  CE &
  0.5530 &
  {\color[HTML]{FE0000} \textbf{3.5121}} &
  \textbf{0.3878} &
  \textbf{0.4070} &
  \multicolumn{1}{c:}{\textbf{0.2923}} &
  -0.0543 &
  {\color[HTML]{000000} -1.1096} &
  0.1514 &
  -0.0971 &
  - 0.0667 \\
\multirow{-7}{*}{ViT} &
  \cellcolor[HTML]{EFEFEF}CE+QR(Ours) &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.6363}} &
  \cellcolor[HTML]{F2F2F2}2.0467 &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.4565}} &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.5024}} &
  \multicolumn{1}{c:}{\cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.3890}}} &
  \cellcolor[HTML]{EFEFEF}0.1280 &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{10.9628}} &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.5306}} &
  \cellcolor[HTML]{EFEFEF}0.1200 &
  \cellcolor[HTML]{EFEFEF}0.0933 \\ \hline
\end{tabular}}

==> Tabels/GI_table.tex <==


%\centering
%\fontsize{8}{9}\selectfont{
%\begin{tabular}{cccccccccc}
%\hline
% &
%   &
%  \multicolumn{4}{c}{\textbf{GILON}} &
%  \multicolumn{4}{c}{\textbf{MS}} \\ \cline{3-10} 
%\multirow{-2}{*}{\textbf{Models}} &
%  \multirow{-2}{*}{\textbf{Methods}} &
%  \textbf{ABC($\uparrow$)} &
%  \textbf{WDACC($\uparrow$)} &
%  \textbf{$\rho_{\text{S}}(\uparrow)$} &
%  \multicolumn{1}{c:}{\textbf{$\rho_{\text{K}}(\uparrow)$}} &
%  \textbf{ABC($\uparrow$)} &
%  \textbf{WDACC($\uparrow$)} &
%  \textbf{$\rho_{\text{S}}(\uparrow)$} &
%  \textbf{$\rho_{\text{K}}(\uparrow)$} \\ \hline
% &
%  GS &
%  0.1524 &
%  0.1954 &
%  0.1051 &
%  \multicolumn{1}{c:}{0.0813} &
%  -0.1591 &
%  0.1668 &
%  0.0514 &
%  \textbf{0.0667} \\
% &
%  SVS &
%  0.8191 &
%  0.3313 &
%  0.1007 &
%  \multicolumn{1}{c:}{0.0681} &
%  0.2253 &
%  0.3291 &
%  -0.0686 &
%  -0.0667 \\
% &
%  Saliency &
%  \textbf{1.1923} &
%  \textbf{0.5467} &
%  {\color[HTML]{FF0000} \textbf{0.3710}} &
%  \multicolumn{1}{c:}{\textbf{0.2571}} &
%  0.0393 &
%  0.1422 &
%  0.1029 &
%  0.1467 \\
% &
%  FA &
%  0.7140 &
%  0.3312 &
%  0.1486 &
%  \multicolumn{1}{c:}{0.1077} &
%  {\color[HTML]{FF0000} \textbf{0.4919}} &
%  0.2876 &
%  -0.0914 &
%  -0.0400 \\
% &
%  IG &
%  0.2100 &
%  0.1934 &
%  0.0457 &
%  \multicolumn{1}{c:}{0.0330} &
%  -0.0157 &
%  0.2410 &
%  \textbf{0.0743} &
%  \textbf{0.0667} \\
% &
%  CE &
%  0.6846 &
%  0.4786 &
%  0.2070 &
%  \multicolumn{1}{c:}{0.1429} &
%  0.3552 &
%  {\color[HTML]{FF0000} \textbf{0.4757}} &
%  0.0629 &
%  0.0133 \\
%\multirow{-7}{*}{ShuffleNet} &
%  \cellcolor[HTML]{EFEFEF}CE+QR(Ours) &
%  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{1.2270}} &
%  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.7607}} &
%  \cellcolor[HTML]{EFEFEF}\textbf{0.3525} &
%  \multicolumn{1}{c:}{\cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.2703}}} &
%  \cellcolor[HTML]{EFEFEF}\textbf{0.3376} &
%  \cellcolor[HTML]{EFEFEF}\textbf{0.4505} &
%  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.6400}} &
%  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.5467}} \\ \hline
% &
%  GS &
%  1.2847 &
%  {\color[HTML]{FF0000} \textbf{0.6716}} &
%  \textbf{0.4532} &
%  \multicolumn{1}{c:}{\textbf{0.3187}} &
%  0.0595 &
%  \textbf{0.3563} &
%  0.0514 &
%  0.0133 \\
% &
%  SVS &
%  0.5772 &
%  0.2812 &
%  0.1341 &
%  \multicolumn{1}{c:}{0.1165} &
%  0.1600 &
%  0.3443 &
%  \textbf{0.3600} &
%  \textbf{0.2800} \\
% &
%  Saliency &
%  {\color[HTML]{FF0000} \textbf{1.3389}} &
%  \textbf{0.6631} &
%  0.3644 &
%  \multicolumn{1}{c:}{0.2879} &
%  0.1542 &
%  0.3455 &
%  0.2514 &
%  0.2000 \\
% &
%  FA &
%  0.8476 &
%  0.4409 &
%  -0.0145 &
%  \multicolumn{1}{c:}{- 0.0242} &
%  {\color[HTML]{FF0000} \textbf{0.3507}} &
%  {\color[HTML]{FF0000} \textbf{0.3732}} &
%  0.1086 &
%  0.0667 \\
% &
%  IG &
%  \textbf{1.2895} &
%  0.6204 &
%  \textbf{0.4532} &
%  \multicolumn{1}{c:}{\textbf{0.3187}} &
%  -0.0058 &
%  0.2443 &
%  0.0514 &
%  0.0133 \\
% &
%  CE &
%  0.8010 &
%  0.4204 &
%  0.3705 &
%  \multicolumn{1}{c:}{0.2703} &
%  \textbf{0.1758} &
%  0.0077 &
%  -0.0629 &
%  -0.0667 \\
%\multirow{-7}{*}{ResNet} &
%  \cellcolor[HTML]{EFEFEF}CE+QR(Ours) &
%  \cellcolor[HTML]{EFEFEF}1.1636 &
%  \cellcolor[HTML]{EFEFEF}0.6150 &
%  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.5815}} &
%  \multicolumn{1}{c:}{\cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.4418}}} &
%  \cellcolor[HTML]{EFEFEF}0.1179 &
%  \cellcolor[HTML]{EFEFEF}0.2544 &
%  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.4400}} &
%  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.3333}} \\ \hline
% &
%  GS &
%  -0.3077 &
%  0.1122 &
%  0.2308 &
%  \multicolumn{1}{c:}{0.1560} &
%  0.2949 &
%  0.2187 &
%  -0.0400 &
%  0.0133 \\
% &
%  SVS &
%  -0.7084 &
%  0.0632 &
%  0.1648 &
%  \multicolumn{1}{c:}{0.1121} &
%  {\color[HTML]{FF0000} \textbf{0.3286}} &
%  0.2261 &
%  -0.1371 &
%  -0.1200 \\
% &
%  Saliency &
%  0.9861 &
%  0.4908 &
%  {\color[HTML]{FF0000} \textbf{0.5253}} &
%  \multicolumn{1}{c:}{{\color[HTML]{FF0000} \textbf{0.4110}}} &
%  0.3216 &
%  \textbf{0.2634} &
%  \textbf{0.0400} &
%  \textbf{0.0400} \\
% &
%  FA &
%  0.4570 &
%  0.2698 &
%  -0.0651 &
%  \multicolumn{1}{c:}{-0.0462} &
%  0.3005 &
%  0.2260 &
%  -0.0457 &
%  -0.0133 \\
% &
%  IG &
%  -0.3012 &
%  0.1157 &
%  0.2352 &
%  \multicolumn{1}{c:}{0.1692} &
%  \textbf{0.3263} &
%  \textbf{0.2631} &
%  -0.0400 &
%  0.0133 \\
% &
%  CE &
%  \textbf{0.9202} &
%  \textbf{0.5312} &
%  \textbf{0.3305} &
%  \multicolumn{1}{c:}{\textbf{0.2396}} &
%  0.1257 &
%  0.1653 &
%  -0.1429 &
%  -0.0933 \\
%\multirow{-7}{*}{MLP-Mixer} &
%  \cellcolor[HTML]{EFEFEF}CE+QR(Ours) &
%  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{1.1442}} &
%  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.6975}} &
%  \cellcolor[HTML]{EFEFEF}0.1657 &
%  \multicolumn{1}{c:}{\cellcolor[HTML]{EFEFEF}0.1297} &
%  \cellcolor[HTML]{EFEFEF}0.2763 &
%  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.2890}} &
%  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.9086}} &
%  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.8133}} \\ \hline
% &
%  GS &
%  -0.1973 &
%  0.1161 &
%  0.2185 &
%  \multicolumn{1}{c:}{0.1473} &
%  \textbf{0.1690} &
%  0.3615 &
%  {\color[HTML]{FF0000} \textbf{0.3600}} &
%  {\color[HTML]{FF0000} \textbf{0.2800}} \\
% &
%  SVS &
%  -0.6079 &
%  0.0839 &
%  0.1314 &
%  \multicolumn{1}{c:}{0.0813} &
%  {\color[HTML]{FF0000} \textbf{0.1821}} &
%  0.3186 &
%  -0.0400 &
%  -0.0667 \\
% &
%  Saliency &
%  \textbf{0.5871} &
%  0.3764 &
%  0.1204 &
%  \multicolumn{1}{c:}{0.0989} &
%  0.1227 &
%  0.3291 &
%  0.0514 &
%  0.0400 \\
% &
%  FA &
%  0.2449 &
%  0.2230 &
%  - 0.0541 &
%  \multicolumn{1}{c:}{-0.0242} &
%  {\color[HTML]{FF0000} \textbf{0.1821}} &
%  0.3186 &
%  0.1429 &
%  0.1200 \\
% &
%  IG &
%  -0.1767 &
%  0.1199 &
%  0.2004 &
%  \multicolumn{1}{c:}{0.1385} &
%  0.1690 &
%  0.3615 &
%  \textbf{0.1771} &
%  \textbf{0.1733} \\
% &
%  CE &
%  0.5530 &
%  \textbf{0.3878} &
%  \textbf{0.4070} &
%  \multicolumn{1}{c:}{\textbf{0.2923}} &
%  -0.0543 &
%  0.1514 &
%  -0.0971 &
%  - 0.0667 \\
%\multirow{-7}{*}{ViT} &
%  \cellcolor[HTML]{EFEFEF}CE+QR(Ours) &
%  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.6363}} &
%  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.4565}} &
%  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.5024}} &
%  \multicolumn{1}{c:}{\cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.3890}}} &
%  \cellcolor[HTML]{EFEFEF}0.1280 &
%  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.5306}} &
%  \cellcolor[HTML]{EFEFEF}0.1200 &
%  \cellcolor[HTML]{EFEFEF}0.0933 \\ \hline
%\end{tabular}}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\centering
\fontsize{8}{9}\selectfont{
\begin{tabular}{cccccccccc}
\hline
 &
   &
  \multicolumn{4}{c}{\textbf{GILON}} &
  \multicolumn{4}{c}{\textbf{MS}} \\ \cline{3-10} 
\multirow{-2}{*}{\textbf{Models}} &
  \multirow{-2}{*}{\textbf{Methods}} &
  \textbf{ABC($\uparrow$)} &
  \textbf{WDACC($\uparrow$)} &
  \textbf{$\rho_{\text{S}}(\uparrow)$} &
  \multicolumn{1}{c:}{\textbf{$\rho_{\text{K}}(\uparrow)$}} &
  \textbf{ABC($\uparrow$)} &
  \textbf{WDACC($\uparrow$)} &
  \textbf{$\rho_{\text{S}}(\uparrow)$} &
  \textbf{$\rho_{\text{K}}(\uparrow)$} \\ \hline
 &
  \multicolumn{1}{c:}{GS} &
  0.1524 &
  0.1954 &
  0.1051 &
  \multicolumn{1}{c:}{0.0813} &
  -0.1591 &
  0.1668 &
  0.0514 &
  \textbf{0.0667} \\
 &
  \multicolumn{1}{c:}{SVS} &
  0.8191 &
  0.3313 &
  0.1007 &
  \multicolumn{1}{c:}{0.0681} &
  0.2253 &
  0.3291 &
  -0.0686 &
  -0.0667 \\
 &
  \multicolumn{1}{c:}{Saliency} &
  \textbf{1.1923} &
  \textbf{0.5467} &
  {\color[HTML]{FF0000} \textbf{0.3710}} &
  \multicolumn{1}{c:}{\textbf{0.2571}} &
  0.0393 &
  0.1422 &
  0.1029 &
  0.1467 \\
 &
  \multicolumn{1}{c:}{FA} &
  0.7140 &
  0.3312 &
  0.1486 &
  \multicolumn{1}{c:}{0.1077} &
  {\color[HTML]{FF0000} \textbf{0.4919}} &
  0.2876 &
  -0.0914 &
  -0.0400 \\
 &
  \multicolumn{1}{c:}{IG} &
  0.2100 &
  0.1934 &
  0.0457 &
  \multicolumn{1}{c:}{0.0330} &
  -0.0157 &
  0.2410 &
  \textbf{0.0743} &
  \textbf{0.0667} \\
 &
  \multicolumn{1}{c:}{CE} &
  0.6846 &
  0.4786 &
  0.2070 &
  \multicolumn{1}{c:}{0.1429} &
  0.3552 &
  {\color[HTML]{FF0000} \textbf{0.4757}} &
  0.0629 &
  0.0133 \\
\multirow{-7}{*}{ShuffleNet} &
  \multicolumn{1}{c:}{\cellcolor[HTML]{EFEFEF}CE+QR(Ours)} &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{1.2270}} &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.7607}} &
  \cellcolor[HTML]{EFEFEF}\textbf{0.3525} &
  \multicolumn{1}{c:}{\cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.2703}}} &
  \cellcolor[HTML]{EFEFEF}\textbf{0.3376} &
  \cellcolor[HTML]{EFEFEF}\textbf{0.4505} &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.6400}} &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.5467}} \\ \hline
 &
  \multicolumn{1}{c:}{GS} &
  1.2847 &
  {\color[HTML]{FF0000} \textbf{0.6716}} &
  \textbf{0.4532} &
  \multicolumn{1}{c:}{\textbf{0.3187}} &
  0.0595 &
  \textbf{0.3563} &
  0.0514 &
  0.0133 \\
 &
  \multicolumn{1}{c:}{SVS} &
  0.5772 &
  0.2812 &
  0.1341 &
  \multicolumn{1}{c:}{0.1165} &
  0.1600 &
  0.3443 &
  \textbf{0.3600} &
  \textbf{0.2800} \\
 &
  \multicolumn{1}{c:}{Saliency} &
  {\color[HTML]{FF0000} \textbf{1.3389}} &
  \textbf{0.6631} &
  0.3644 &
  \multicolumn{1}{c:}{0.2879} &
  0.1542 &
  0.3455 &
  0.2514 &
  0.2000 \\
 &
  \multicolumn{1}{c:}{FA} &
  0.8476 &
  0.4409 &
  -0.0145 &
  \multicolumn{1}{c:}{- 0.0242} &
  {\color[HTML]{FF0000} \textbf{0.3507}} &
  {\color[HTML]{FF0000} \textbf{0.3732}} &
  0.1086 &
  0.0667 \\
 &
  \multicolumn{1}{c:}{IG} &
  \textbf{1.2895} &
  0.6204 &
  \textbf{0.4532} &
  \multicolumn{1}{c:}{\textbf{0.3187}} &
  -0.0058 &
  0.2443 &
  0.0514 &
  0.0133 \\
 &
  \multicolumn{1}{c:}{CE} &
  0.8010 &
  0.4204 &
  0.3705 &
  \multicolumn{1}{c:}{0.2703} &
  \textbf{0.1758} &
  0.0077 &
  -0.0629 &
  -0.0667 \\
\multirow{-7}{*}{ResNet} &
  \multicolumn{1}{c:}{\cellcolor[HTML]{EFEFEF}CE+QR(Ours)} &
  \cellcolor[HTML]{EFEFEF}1.1636 &
  \cellcolor[HTML]{EFEFEF}0.6150 &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.5815}} &
  \multicolumn{1}{c:}{\cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.4418}}} &
  \cellcolor[HTML]{EFEFEF}0.1179 &
  \cellcolor[HTML]{EFEFEF}0.2544 &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.4400}} &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.3333}} \\ \hline
 &
  \multicolumn{1}{c:}{GS} &
  -0.3077 &
  0.1122 &
  0.2308 &
  \multicolumn{1}{c:}{0.1560} &
  0.2949 &
  0.2187 &
  -0.0400 &
  0.0133 \\
 &
  \multicolumn{1}{c:}{SVS} &
  -0.7084 &
  0.0632 &
  0.1648 &
  \multicolumn{1}{c:}{0.1121} &
  {\color[HTML]{FF0000} \textbf{0.3286}} &
  0.2261 &
  -0.1371 &
  -0.1200 \\
 &
  \multicolumn{1}{c:}{Saliency} &
  0.9861 &
  0.4908 &
  {\color[HTML]{FF0000} \textbf{0.5253}} &
  \multicolumn{1}{c:}{{\color[HTML]{FF0000} \textbf{0.4110}}} &
  0.3216 &
  \textbf{0.2634} &
  \textbf{0.0400} &
  \textbf{0.0400} \\
 &
  \multicolumn{1}{c:}{FA} &
  0.4570 &
  0.2698 &
  -0.0651 &
  \multicolumn{1}{c:}{-0.0462} &
  0.3005 &
  0.2260 &
  -0.0457 &
  -0.0133 \\
 &
  \multicolumn{1}{c:}{IG} &
  -0.3012 &
  0.1157 &
  0.2352 &
  \multicolumn{1}{c:}{0.1692} &
  \textbf{0.3263} &
  \textbf{0.2631} &
  -0.0400 &
  0.0133 \\
 &
  \multicolumn{1}{c:}{CE} &
  \textbf{0.9202} &
  \textbf{0.5312} &
  \textbf{0.3305} &
  \multicolumn{1}{c:}{\textbf{0.2396}} &
  0.1257 &
  0.1653 &
  -0.1429 &
  -0.0933 \\
\multirow{-7}{*}{MLP-Mixer} &
  \multicolumn{1}{c:}{\cellcolor[HTML]{EFEFEF}CE+QR(Ours)} &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{1.1442}} &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.6975}} &
  \cellcolor[HTML]{EFEFEF}0.1657 &
  \multicolumn{1}{c:}{\cellcolor[HTML]{EFEFEF}0.1297} &
  \cellcolor[HTML]{EFEFEF}0.2763 &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.2890}} &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.9086}} &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.8133}} \\ \hline
 &
  \multicolumn{1}{c:}{GS} &
  -0.1973 &
  0.1161 &
  0.2185 &
  \multicolumn{1}{c:}{0.1473} &
  \textbf{0.1690} &
  0.3615 &
  {\color[HTML]{FF0000} \textbf{0.3600}} &
  {\color[HTML]{FF0000} \textbf{0.2800}} \\
 &
  \multicolumn{1}{c:}{SVS} &
  -0.6079 &
  0.0839 &
  0.1314 &
  \multicolumn{1}{c:}{0.0813} &
  {\color[HTML]{FF0000} \textbf{0.1821}} &
  0.3186 &
  -0.0400 &
  -0.0667 \\
 &
  \multicolumn{1}{c:}{Saliency} &
  \textbf{0.5871} &
  0.3764 &
  0.1204 &
  \multicolumn{1}{c:}{0.0989} &
  0.1227 &
  0.3291 &
  0.0514 &
  0.0400 \\
 &
  \multicolumn{1}{c:}{FA} &
  0.2449 &
  0.2230 &
  - 0.0541 &
  \multicolumn{1}{c:}{-0.0242} &
  {\color[HTML]{FF0000} \textbf{0.1821}} &
  0.3186 &
  0.1429 &
  0.1200 \\
 &
  \multicolumn{1}{c:}{IG} &
  -0.1767 &
  0.1199 &
  0.2004 &
  \multicolumn{1}{c:}{0.1385} &
  0.1690 &
  0.3615 &
  \textbf{0.1771} &
  \textbf{0.1733} \\
 &
  \multicolumn{1}{c:}{CE} &
  0.5530 &
  \textbf{0.3878} &
  \textbf{0.4070} &
  \multicolumn{1}{c:}{\textbf{0.2923}} &
  -0.0543 &
  0.1514 &
  -0.0971 &
  - 0.0667 \\
\multirow{-7}{*}{ViT} &
  \multicolumn{1}{c:}{\cellcolor[HTML]{EFEFEF}CE+QR(Ours)} &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.6363}} &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.4565}} &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.5024}} &
  \multicolumn{1}{c:}{\cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.3890}}} &
  \cellcolor[HTML]{EFEFEF}0.1280 &
  \cellcolor[HTML]{EFEFEF}{\color[HTML]{FF0000} \textbf{0.5306}} &
  \cellcolor[HTML]{EFEFEF}0.1200 &
  \cellcolor[HTML]{EFEFEF}0.0933 \\ \hline
\end{tabular}}
